Probabilistic Reach-Avoid for Bayesian Neural Networks

Model-based reinforcement learning seeks to simultaneously learn the dynamics of an unknown stochastic environment and synthesise an optimal policy for acting in it. Ensuring the safety and robustness of sequential decisions made through a policy in such an environment is a key challenge for policies intended for safety-critical scenarios. In this work, we investigate two complementary problems: first, computing reach-avoid probabilities for iterative predictions made with dynamical models, with dynamics described by Bayesian neural network (BNN); second, synthesising control policies that are optimal with respect to a given reach-avoid specification (reaching a "target" state, while avoiding a set of "unsafe" states) and a learned BNN model. Our solution leverages interval propagation and backward recursion techniques to compute lower bounds for the probability that a policy's sequence of actions leads to satisfying the reach-avoid specification. Such computed lower bounds provide safety certification for the given policy and BNN model. We then introduce control synthesis algorithms to derive policies maximizing said lower bounds on the safety probability. We demonstrate the effectiveness of our method on a series of control benchmarks characterized by learned BNN dynamics models. On our most challenging benchmark, compared to purely data-driven policies the optimal synthesis algorithm is able to provide more than a four-fold increase in the number of certifiable states and more than a three-fold increase in the average guaranteed reach-avoid probability.

==> Sections/Methodology_old.tex <==
\section{Synthesizing Robust Strategies}

N.B. this is just a sketch of the methodology I am currently refining. The aim here is just to present the core ideas with some notation to make things easier to discuss

\subsection{Episodic Learning Framework}

As in our previous work, we follow an episodic learning framework to at once fit a model of the dynamics as well as learn a suitable control policy. Each episode three steps first we collect data, second we fit a Bayesian neural network dynamics model, and finally we update our control policy. We assume that the state-space of the control setting of interest occurs in $\mathbb{R}^n$ and that the action space is $\mathbb{R}^{m}$. We define the true transition function $T : \mathbb{R}^{n \times m} \longrightarrow \mathbb{R}^{n}$ to be a mapping that takes in a state and an action and returns the next state. Finally, we assume that their is a set of states $\mathcal{G} \subset \mathbb{R}^{n}$ which are considered the goal region as well as a set of states $\mathcal{O} \subset \mathbb{R}^{n}$  that denote obstacles. The general goal of our episodic learning framework is to learn a Bayesian neural network $f^w \approx T$ and a control policy $\pi$ such that acting according to $\pi$ reaches the goal from anywhere in the state-space while avoiding the obstacles. Below we detail how this is done.

We set up an action matrix $\mathcal{A}$ which is that is a discretized representation of $\mathbb{R}^n$. We denote each dimension of our state-space as being broken into $k_i$ different chunks; thus, $\mathcal{A} \in \mathbb{R}^{n_0 \times \cdots \times k_n \times m}$ where the final $m$ is due to the fact that each entry of our action matrix contains an action. Initially, we set each action to be a random vector selected uniformly at random and then normalized so it has unit $\ell_2$ norm. Given this matrix, we can map any vector $s \in \mathbb{R}^n$ to its corresponding action by simply rounding the $i^{th}$ entry of $s$ to the nearest $1/k_i$ for each $i$. When accessing values of this matrix we will simply denote the entry in square brackets We can then simulate the result of following the policy according to the environment in the following way: 

\begin{align}
    s^{index}_i &= round(s_i)\\
    a_{i} &= \mathcal{A}[s_i^{index}]\\
    s_{i+1} &= T(s_{i}, a_{i})
\end{align}

The first step of our episodic learning framework consists of simply randomly sampling $q$-many random states, and simulating forward $t$ time steps forward according to the equations above. In doing so, we build a dynamics dataset $\mathcal{D} := \{ (s_i, a_i), s_{i+1} \}_{i=0}^{t\times q}$. 

Given this dataset, we can proceed to the next step of our framework. Given a neural network architecture $f$ parameterized by weights $w$, we use Bayes rule to infer a distribution over the weights of a neural network thus yielding a Bayesian neural network. This is done by considering the state-action pairs as inputs $x \in \mathbb{R}^{n \times m}$ and their resulting states as outputs $y \in \mathbb{R}^{n}$. Given the dataset of these values $X = \{x_i\}_{i=0}^{t\times q}$, $Y = \{y_i\}_{i=0}^{t\times q}$ observed from acting according to $\mathcal{A}$ we can infer weights according to the following rule: 

\begin{align}
    p(w | X, Y) \propto p(Y | X, w) p(w)
\end{align}

Given $p(w | X, Y)$, we can perform inference for what we believe the next state will be according to the posterior predictive distribution: 

\begin{align}
    p(y | x, X, Y) = p(y | x, w) p(w | X, Y)
\end{align}

For convenience we will use $f^w(x)$ in place of the predictive distribution. The benefit of this distribution is that we use this in place of equation (3) above: $\hat{s}_{i+1} = f^{w}(s_i, a_i)$.

Before recollecting data, we need to update our action matrix in order to reflect our beliefs about how to best act. We do so by esablishing a loss function $\mathcal{L} : \mathbb{R}^{n \times m} \longrightarrow \mathbb{R}$ which scores (as a real value) how good or bad the result of applying action $a$ in state $s$ with good values being larger. The loss function is constructed in practice using the state location of obstacles, attractors and the goal region. An action $a$ is rewarded if it moves towards attractors and the goal region and is penalized for moving towards obstacles. When updating $\mathcal{A}$, our goal is to solve the following optimization problem: 

\begin{align}
    a^{*} = \argmax_{a} \mathcal{L}(s, a)
\end{align}

for each entry of the action matrix. We solve this by stochastic gradient descent (thus yielding a maximum likelihood solution). Finally, we re-collect data by acting in the real environment (according to $T$) with this new action matrix. 


\subsection{Synthesizing Certifiable/Optimal $\mathcal{A}$}

In practice, the action matrix we learn may not be optimally certifiable. Though in our previous work we show how to certify an arbitrary policy $\pi$, in this work we are interested in further learning the best such $\pi$. (We attempted this briefly in the original paper, but not with any guarantees).

The sketch of the idea is to perform as follows: during the backwards reachability procedure from the previous paper rather than taking the action as a give, we test a series of $\tau$ actions in a grid. For each action, we compute the reach-avoid probability and then we take the action with the highest probability to be the action in the action matrix $\mathcal{A}$. Given that we have sampled enough actions we can easily have guarantees that the selected action is a bounded distance from the action which truly maximizes the reachability probability according to our posterior beliefs. 
